GWTC-4.0: Searches for Gravitational-Wave Lensing Signatures

Gravitational waves can be gravitationally lensed by massive objects along their path. Depending on the lens mass and the lens--source geometry, this can lead to the observation of a single distorted signal or multiple repeated events with the same frequency evolution. We present the results for gravitational-wave lensing searches on the data from the first part of the fourth LIGO--Virgo--KAGRA observing run (O4a). We search for strongly lensed events in the newly acquired data by (1) searching for an overall phase shift present in an image formed at a saddle point of the lens potential, (2) looking for pairs of detected candidates with consistent frequency evolution, and (3) identifying sub-threshold counterpart candidates to the detected signals. Beyond strong lensing, we also look for lensing-induced distortions in all detected signals using an isolated point-mass model. We do not find evidence for strongly lensed gravitational-wave signals and use this result to constrain the rate of detectable strongly lensed events and the merger rate density of binary black holes at high redshift. In the search for single distorted lensed signals, we find one outlier: GW231123_135430, for which we report more detailed investigations. While this event is interesting, the associated waveform uncertainties make its interpretation complicated, and future observations of the populations of binary black holes and of gravitational lenses will help determine the probability that this event could be lensed.

==> gwtc-4-common-files/LVKack.tex <==
This material is based upon work supported by NSF’s LIGO Laboratory which is a major facility
fully funded by the National Science Foundation.
The authors also gratefully acknowledge the support of
% the United States National Science Foundation (NSF) for the construction and operation of the
% LIGO Laboratory and Advanced LIGO as well as
the Science and Technology Facilities Council (STFC) of the
United Kingdom, the Max-Planck-Society (MPS), and the State of
Niedersachsen/Germany for support of the construction of Advanced LIGO 
and construction and operation of the GEO\,600 detector. 
Additional support for Advanced LIGO was provided by the Australian Research Council.
The authors gratefully acknowledge the Italian Istituto Nazionale di Fisica Nucleare (INFN),  
the French Centre National de la Recherche Scientifique (CNRS) and
the Netherlands Organization for Scientific Research, 
for the construction and operation of the Virgo detector
and the creation and support  of the EGO consortium. 
The authors also gratefully acknowledge research support from these agencies as well as by 
the Council of Scientific and Industrial Research of India, 
the Department of Science and Technology, India,
the Science \& Engineering Research Board (SERB), India,
the Ministry of Human Resource Development, India,
the Spanish Agencia Estatal de Investigaci\'on,
the Vicepresid\`encia i Conselleria d'Innovaci\'o, Recerca i Turisme and the Conselleria d'Educaci\'o i Universitat del Govern de les Illes Balears,
the Conselleria d'Innovaci\'o, Universitats, Ci\`encia i Societat Digital de la Generalitat Valenciana and
the CERCA Programme Generalitat de Catalunya, Spain,
the National Science Centre of Poland and the Foundation for Polish Science (FNP),
the Swiss National Science Foundation (SNSF),
the Russian Foundation for Basic Research, 
the Russian Science Foundation,
the European Commission,
the European Regional Development Funds (ERDF),
the Royal Society, 
the Scottish Funding Council, 
the Scottish Universities Physics Alliance, 
the Hungarian Scientific Research Fund (OTKA),
the French Lyon Institute of Origins (LIO),
the Belgian Fonds de la Recherche Scientifique (FRS-FNRS), 
Actions de Recherche Concertées (ARC) and
Fonds Wetenschappelijk Onderzoek – Vlaanderen (FWO), Belgium,
the Paris \^{I}le-de-France Region, 
the National Research, Development and Innovation Office Hungary (NKFIH), 
the National Research Foundation of Korea,
the Natural Science and Engineering Research Council Canada,
Canadian Foundation for Innovation (CFI),
the Brazilian Ministry of Science, Technology, and Innovations,
the International Center for Theoretical Physics South American Institute for Fundamental Research (ICTP-SAIFR), 
the Research Grants Council of Hong Kong,
the National Natural Science Foundation of China (NSFC),
the Leverhulme Trust, 
the Research Corporation, 
the Ministry of Science and Technology (MOST), Taiwan,
the United States Department of Energy,
and
the Kavli Foundation.
The authors gratefully acknowledge the support of the NSF, STFC, INFN and CNRS for provision of computational resources.
Computing was performed on the OzSTAR Australian national facility at Swinburne University of Technology, which receives funding in part from the Astronomy National Collaborative Research Infrastructure Strategy (NCRIS) allocation provided by the Australian Government.
We thankfully acknowledge the computer resources at MareNostrum and the technical support provided by Barcelona Supercomputing Center (RES-AECT-2021-2-0021). 
This work was supported by MEXT, JSPS Leading-edge Research Infrastructure Program, JSPS Grant-in-Aid for Specially Promoted Research 26000005, JSPS Grant-in-Aid for Scientific Research on Innovative Areas 2905: JP17H06358, JP17H06361 and JP17H06364, JSPS Core-to-Core Program A.\ Advanced Research Networks, JSPS Grant-in-Aid for Scientific Research (S) 17H06133, the joint research program of the Institute for Cosmic Ray Research, University of Tokyo, National Research Foundation (NRF) and Computing Infrastructure Project of KISTI-GSDC in Korea, Academia Sinica (AS), AS Grid Center (ASGC) and the Ministry of Science and Technology (MoST) in Taiwan under grants including AS-CDA-105-M06, Advanced Technology Center (ATC) of NAOJ, and Mechanical Engineering Center of KEK.




==> gwtc-4-common-files/macros/misc_macros.tex <==
% Software styling
\newcommand{\soft}[1]{\textsc{#1}}

% Stylized software names
\newcommand{\GSTLAL}{\soft{GstLAL}\xspace}
\newcommand{\BAYESTAR}{\soft{BAYESTAR}\xspace}
\newcommand{\CWB}{\soft{CWB}\xspace}
\newcommand{\PYCBC}{\soft{PyCBC}\xspace}
\newcommand{\MBTA}{\soft{MBTA}\xspace}
\newcommand{\SPIIR}{\soft{SPIIR}\xspace}
\newcommand{\LALINFERENCE}{\soft{LALInference}\xspace}
\newcommand{\BAYESWAVE}{\soft{BayesWave}\xspace}
\newcommand{\BILBY}{\soft{Bilby}\xspace}
\newcommand{\RIFT}{\soft{RIFT}\xspace}
\newcommand{\LALSUITE}{\soft{LALSuite}\xspace}
\newcommand{\BILBYPIPE}{\soft{BilbyPipe}\xspace}
\newcommand{\PBILBY}{\soft{ParallelBilby}\xspace}
\newcommand{\ASIMOV}{\soft{Asimov}\xspace}
\newcommand{\PESUMMARY}{\soft{PESummary}\xspace}
\newcommand{\PYTHON}{\soft{Python}\xspace}
\newcommand{\NUMPY}{\soft{NumPy}\xspace}
\newcommand{\SCIPY}{\soft{SciPy}\xspace}
\newcommand{\MATPLOTLIB}{\soft{Matplotlib}\xspace}
\newcommand{\SEABORN}{\soft{seaborn}\xspace}
\newcommand{\GWPY}{\soft{GWpy}\xspace}
\newcommand{\DYNESTY}{\soft{Dynesty}\xspace}


==> gwtc-4-common-files/macros/quantities_macros.tex <==
%% THIS FILE IS AUTOGENERATED - DO NOT EDIT
\providecolor{UNREVIEWED}{rgb}{1,0,0}
\providecolor{REVIEWED}{rgb}{0,.5,.5}


\DeclareSIUnit\parsec{pc}
\DeclareSIUnit\Mpc{\mega\parsec}

\newcommand{\OoneLHORange}{{\color{UNREVIEWED}{\qty{80.0}{\Mpc}}}}
\newcommand{\OoneLLORange}{{\color{UNREVIEWED}{\qty{70.0}{\Mpc}}}}
\newcommand{\OtwoLHORange}{{\color{UNREVIEWED}{\qty{70.0}{\Mpc}}}}
\newcommand{\OtwoLLORange}{{\color{UNREVIEWED}{\qty{100.0}{\Mpc}}}}
\newcommand{\OtwoVirgoRange}{{\color{UNREVIEWED}{\qty{30.0}{\Mpc}}}}
\newcommand{\OthreeaLHORange}{{\color{UNREVIEWED}{\qty{120.0}{\Mpc}}}}
\newcommand{\OthreeaLLORange}{{\color{UNREVIEWED}{\qty{140.0}{\Mpc}}}}
\newcommand{\OthreeaVirgoRange}{{\color{UNREVIEWED}{\qty{50.0}{\Mpc}}}}
\newcommand{\OthreebLHORange}{{\color{UNREVIEWED}{\qty{120.0}{\Mpc}}}}
\newcommand{\OthreebLLORange}{{\color{UNREVIEWED}{\qty{140.0}{\Mpc}}}}
\newcommand{\OthreebVirgoRange}{{\color{UNREVIEWED}{\qty{60.0}{\Mpc}}}}
\newcommand{\OthreeGKKagraRange}{{\color{UNREVIEWED}{\qty{0.7}{\Mpc}}}}
\newcommand{\OthreeGKGeoRange}{{\color{UNREVIEWED}{\qty{1.1}{\Mpc}}}}
\newcommand{\OthreeLHORange}{{\color{UNREVIEWED}{\qty{120.0}{\Mpc}}}}
\newcommand{\OthreeLLORange}{{\color{UNREVIEWED}{\qty{140.0}{\Mpc}}}}
\newcommand{\OthreeVirgoRange}{{\color{UNREVIEWED}{\qty{50.0}{\Mpc}}}}
\newcommand{\OfouraLHORange}{{\color{UNREVIEWED}{\qty{150.0}{\Mpc}}}}
\newcommand{\OfouraLLORange}{{\color{UNREVIEWED}{\qty{160.0}{\Mpc}}}}

